Space-time multilevel Monte Carlo methods and their application to cardiac electrophysiology

We present a novel approach aimed at high-performance uncertainty quantification for time-dependent problems governed by partial differential equations. In particular, we consider input uncertainties described by a Karhunen-Loeeve expansion and compute statistics of high-dimensional quantities-of-interest, such as the cardiac activation potential. Our methodology relies on a close integration of multilevel Monte Carlo methods, parallel iterative solvers, and a space-time discretization. This combination allows for space-time adaptivity, time-changing domains, and to take advantage of past samples to initialize the space-time solution. The resulting sequence of problems is distributed using a multilevel parallelization strategy, allocating batches of samples having different sizes to a different number of processors. We assess the performance of the proposed framework by showing in detail its application to the solution of nonlinear equations arising from cardiac electrophysiology. Specifically, we study the effect of spatially-correlated perturbations of the heart fibers conductivities on the mean and variance of the resulting activation map. As shown by the experiments, the theoretical rates of convergence of multilevel Monte Carlo are achieved. Moreover, the total computational work for a prescribed accuracy is reduced by an order of magnitude with respect to standard Monte Carlo methods.

==> not_needed <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Alessio Quaglino at 2018-05-03 09:31:10 +0200 


%% Saved with string encoding Unicode (UTF-8) 


@comment{jabref-meta: databaseType:bibtex;}



@misc{quaglino2017sloth,
	Author = {Quaglino, Alessio, Ben Bader, Seif and Krause, Rolf},
	Date-Added = {2018-05-03 07:30:52 +0000},
	Date-Modified = {2018-05-03 07:31:10 +0000},
	Howpublished = {software},
	Title = {SLOTH: A Python library for UQ},
	Year = {2017}}

@techreport{pisaroni2017quantifying,
	Author = {Pisaroni, Michele and Krumscheid, Sebastian and Nobile, Fabio},
	Date-Added = {2018-04-13 07:37:53 +0000},
	Date-Modified = {2018-04-13 07:37:53 +0000},
	Title = {Quantifying uncertain system outputs via the multilevel {Monte Carlo} method--{Part I}: {C}entral moment estimation},
	Year = {2017}}

@article{bierig2015convergence,
	Author = {Bierig, Claudio and Chernov, Alexey},
	Date-Added = {2018-04-13 07:37:31 +0000},
	Date-Modified = {2018-04-13 07:37:31 +0000},
	Journal = {Numerische Mathematik},
	Number = {4},
	Pages = {579--613},
	Publisher = {Springer},
	Title = {Convergence analysis of multilevel {Monte Carlo} variance estimators and application for random obstacle problems},
	Volume = {130},
	Year = {2015}}

@article{biehler2017impact,
	Author = {Biehler, J and Wall, WA},
	Date-Added = {2017-10-11 07:38:30 +0000},
	Date-Modified = {2017-10-11 07:38:30 +0000},
	Journal = {International Journal for Numerical Methods in Biomedical Engineering},
	Publisher = {Wiley Online Library},
	Title = {The impact of personalized probabilistic wall thickness models on peak wall stress in abdominal aortic aneurysms},
	Year = {2017}}

@article{koutsourelakis2009accurate,
	Author = {Koutsourelakis, Phaedon-Stelios},
	Journal = {SIAM J. Sci. Comput.},
	Number = {5},
	Pages = {3274--3300},
	Publisher = {SIAM},
	Title = {Accurate uncertainty quantification using inaccurate computational models},
	Volume = {31},
	Year = {2009}}

@article{mirams2016,
	Author = {Mirams, Gary R. and Pathmanathan, Pras and Gray, Richard A. and Challenor, Peter and Clayton, Richard H.},
	Doi = {10.1113/JP271671},
	Issn = {1469-7793},
	Journal = {The Journal of Physiology},
	Number = {23},
	Pages = {6833--6847},
	Title = {Uncertainty and variability in computational and mathematical models of cardiac physiology},
	Url = {http://dx.doi.org/10.1113/JP271671},
	Volume = {594},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1113/JP271671}}

@article{richardson2011,
	Author = {Richardson, Giles and Chapman, S Jonathan},
	Journal = {SIAM J. Appl. Math.},
	Number = {3},
	Pages = {657--675},
	Publisher = {SIAM},
	Title = {Derivation of the bidomain equations for a beating heart with a general microstructure},
	Volume = {71},
	Year = {2011}}

@article{sanchez2017,
	Author = {S{\'a}nchez, Carlos and D'Ambrosio, Gabriele and Maffessanti, Francesco and Caiani, Enrico and Prinzen, Frits and Krause, Rolf and Auricchio, Angelo and Potse, Mark},
	Journal = {Med Biol Eng Comput.},
	Title = {Sensitivity Analysis of Ventricular Activation and Electrocardiogram in Tailored Models of Heart-Failure Patients},
	Year = {2017}}

@article{niederer2011,
	Author = {Niederer, Steven and Mitchell, Lawrence and Smith, Nicolas and Plank, Gernot},
	Journal = {Front. Physiol.},
	Publisher = {Frontiers Media SA},
	Title = {Simulating human cardiac electrophysiology on clinical time-scales},
	Volume = {2},
	Year = {2011}}

@article{colli93,
	Author = {{Colli Franzone}, Piero and Guerri, Luciano},
	Doi = {10.1016/0025-5564(93)90001-q},
	Journal = {Math. Biosci.},
	Pages = {145--209},
	Title = {Spreading of Excitation in {3-D} Models of the Anisotropic Cardiac Tissue. {I}. Validation of the Eikonal Model},
	Volume = {113},
	Year = {1993},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/0025-5564(93)90001-q}}

@article{pullan2002,
	Author = {Andrew J. Pullan and Karl A. Tomlinson and Peter J. Hunter},
	Doi = {10.1137/S0036139901389513},
	Journal = {SIAM J. Appl. Math.},
	Number = {1},
	Pages = {324-350},
	Title = {A Finite Element Method for an Eikonal Equation Model of Myocardial Excitation Wavefront Propagation},
	Url = {http://dx.doi.org/10.1137/S0036139901389513},
	Volume = {63},
	Year = {2002},
	Bdsk-Url-1 = {http://dx.doi.org/10.1137/S0036139901389513}}

@article{pezzuto2017,
	Abstract = {State-of-the-art cardiac electrophysiology models
                   that are able to deliver physiologically motivated
                   activation maps and electrocardiograms (ECGs) can
                   only be solved on high-performance computing
                   architectures. This makes it nearly impossible to
                   adopt such models in clinical practice. ECG imaging
                   tools typically rely on simplified models, but these
                   neglect the anisotropic electric conductivity of the
                   tissue in the forward problem. Moreover, their
                   results are often confined to the heart-torso
                   interface. We propose a forward model that fully
                   accounts for the anisotropic tissue conductivity and
                   produces the standard 12-lead ECG in a few seconds.
                   The activation sequence is approximated with an
                   eikonal model in the 3d myocardium, while the ECG is
                   computed with the lead-field approach. Both solvers
                   were implemented on graphics processing units and
                   massively parallelized. We studied the numerical
                   convergence and scalability of the approach. We also
                   compared the method to the bidomain model in terms of
                   ECGs and activation maps, using a simplified but
                   physiologically motivated geometry and 6
                   patient-specific anatomies. The proposed methods
                   provided a good approximation of activation maps and
                   ECGs computed with a bidomain model, in only a few
                   seconds. Both solvers scaled very well to high-end
                   hardware. These methods are suitable for use in ECG
                   imaging methods, and may soon become fast enough for
                   use in interactive simulation tools.},
	Author = {Pezzuto, Simone and Kal'avsk{\'y}, Peter and Potse, Mark and Prinzen, Frits W and Auricchio, Angelo and Krause, Rolf},
	Doi = {10.3389/fphys.2017.00265},
	Issn = {1664-042X},
	Journal = {Front. Physiol.},
	Pages = {265},
	Title = {Evaluation of a Rapid Anisotropic Model for {ECG} Simulation.},
	Volume = {8},
	Year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.3389/fphys.2017.00265}}

@article{corrado2015identification,
	Author = {Corrado, Cesare and Gerbeau, Jean-Fr{\'e}d{\'e}ric and Moireau, Philippe},
	Journal = {J. Comput. Phys.},
	Pages = {271--298},
	Publisher = {Elsevier},
	Title = {Identification of weakly coupled multiphysics problems. Application to the inverse problem of electrocardiography},
	Volume = {283},
	Year = {2015}}

@article{gilesmultilevel,
	Author = {Giles, Michael B.},
	Doi = {10.1017/S096249291500001X},
	Journal = {Acta Numerica},
	Pages = {259---328},
	Publisher = {Cambridge University Press},
	Title = {Multilevel {Monte Carlo} methods},
	Volume = {24},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1017/S096249291500001X}}

@article{biehler2015towards,
	Author = {Biehler, Jonas and Gee, Michael W and Wall, Wolfgang A},
	Journal = {Biomech. Model. Mechanobiol.},
	Number = {3},
	Pages = {489--513},
	Publisher = {Springer},
	Title = {Towards efficient uncertainty quantification in complex and large-scale biomechanical problems based on a Bayesian multi-fidelity scheme},
	Volume = {14},
	Year = {2015}}

@inproceedings{baker2002dynamic,
	Author = {Baker, Timothy J and Pebay, P and Pousin, J{\'e}r{\^o}me},
	Booktitle = {WCCM V-Fifth World Congress on Computational Mechanics, Vienna},
	Title = {Dynamic meshing for finite element based segmentation of cardiac imagery},
	Year = {2002}}

@article{peherstorfer2015optimal,
	Author = {Peherstorfer, Benjamin and Willcox, Karen and Gunzburger, Max},
	Doi = {10.1137/15m1046472},
	Institution = {SIAM Journal on Scientific Computing},
	Journal = {{SIAM} Journal on Scientific Computing},
	Month = {jan},
	Number = {5},
	Pages = {A3163--A3194},
	Publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
	Title = {Optimal model management for multifidelity {Monte Carlo} estimation},
	Volume = {38},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1137/15m1046472}}


@article{peherstorfer2016survey,
  title={Survey of multifidelity methods in uncertainty propagation, inference, and optimization},
  author={Peherstorfer, Benjamin and Willcox, Karen and Gunzburger, Max},
  journal={Siam Review},
  volume={60},
  number={3},
  pages={550--591},
  year={2018},
  publisher={SIAM}
}

@article{reinert2006including,
	Author = {Reinert, Joshua M and Apostolakis, George E},
	Journal = {Ann. Nucl. Energy},
	Number = {4},
	Pages = {354--369},
	Publisher = {Elsevier},
	Title = {Including model uncertainty in risk-informed decision making},
	Volume = {33},
	Year = {2006}}

@article{leifsson2010multi,
	Author = {Leifsson, Leifur and Koziel, Slawomir},
	Journal = {Journal of Computational Science},
	Number = {2},
	Pages = {98--106},
	Publisher = {Elsevier},
	Title = {Multi-fidelity design optimization of transonic airfoils using physics-based surrogate modeling and shape-preserving response prediction},
	Volume = {1},
	Year = {2010}}

@book{colli14,
	Author = {Colli Franzone, Piero and Pavarino, Luca F. and Scacchi, Simone},
	Doi = {10.1007/978-3-319-04801-7},
	Publisher = {Springer},
	Title = {Mathematical Cardiac Electrophysiology},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/978-3-319-04801-7}}

@article{dierckx2011,
	Author = {Dierckx, Hans and Bernus, Olivier and Verschelde, Henri},
	Doi = {10.1103/PhysRevLett.107.108101},
	Journal = {Phys. Rev. Lett.},
	Number = {10},
	Pages = {108101},
	Publisher = {APS},
	Title = {Accurate eikonal-curvature relation for wave fronts in locally anisotropic reaction-diffusion systems},
	Volume = {107},
	Year = {2011},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevLett.107.108101}}

@article{jeong2008,
	Author = {Jeong, Won-Ki and Whitaker, Ross T},
	Doi = {10.1137/060670298},
	Journal = {SIAM J. Sci. Comput.},
	Number = {5},
	Pages = {2512--2534},
	Publisher = {SIAM},
	Title = {A fast iterative method for eikonal equations},
	Volume = {30},
	Year = {2008},
	Bdsk-Url-1 = {http://dx.doi.org/10.1137/060670298}}

@article{bornemann2006,
	Author = {Bornemann, Folkmar and Rasch, Christian},
	Doi = {10.1007/s00791-006-0016-y},
	Issn = {1432-9360},
	Journal = {Computing and Visualization in Science},
	Language = {english},
	Number = {2},
	Pages = {57-69},
	Publisher = {Springer-Verlag},
	Title = {Finite-element Discretization of Static {Hamilton}-{Jacobi} Equations based on a Local Variational Principle},
	Url = {http://dx.doi.org/10.1007/s00791-006-0016-y},
	Volume = {9},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s00791-006-0016-y}}

@article{potse2006,
	Author = {Potse, Mark and Dub{\'e}, Bruno and Richer, Jacques and Vinet, Alain and Gulrajani, Ramesh M.},
	Journal = {IEEE Trans. Biomed. Eng.},
	Number = {12},
	Pages = {2425-2435},
	Title = {A Comparison of monodomain and bidomain {\hbox{reaction-diffusion}} models for action potential propagation in the human heart},
	Volume = {53},
	Year = {2006}}

@article{streeter1969,
	Author = {Streeter, Daniel D and Spotnitz, Henry M and Patel, Dali P and Ross, John and Sonnenblick, Edmund H},
	Doi = {10.1161/01.res.24.3.339},
	Journal = {Circ. Res.},
	Number = {3},
	Pages = {339--347},
	Publisher = {Am Heart Assoc},
	Title = {Fiber orientation in the canine left ventricle during diastole and systole},
	Volume = {24},
	Year = {1969},
	Bdsk-Url-1 = {http://dx.doi.org/10.1161/01.res.24.3.339}}

@article{beyar1984,
	Author = {Beyar, R and Sideman, S},
	Journal = {Circ. Res.},
	Number = {3},
	Pages = {358--375},
	Publisher = {Am Heart Assoc},
	Title = {A computer study of the left ventricular performance based on fiber structure, sarcomere dynamics, and transmural electrical propagation velocity.},
	Volume = {55},
	Year = {1984}}

@article{harbrecht2012,
	Author = {Harbrecht, Helmut and Peters, Michael and Schneider, Reinhold},
	Doi = {10.1016/j.apnum.2011.10.001},
	Journal = {Applied numerical mathematics},
	Number = {4},
	Pages = {428--440},
	Publisher = {Elsevier},
	Title = {On the low-rank approximation by the pivoted {Cholesky} decomposition},
	Volume = {62},
	Year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.apnum.2011.10.001}}

@article{potse2012,
	Author = {Potse, Mark and Krause, Dorian and Bacharova, Ljuba and Krause, Rolf and Prinzen, Frits W and Auricchio, Angelo},
	Journal = {Europace},
	Number = {suppl\_5},
	Pages = {v33--v39},
	Publisher = {Oxford University Press},
	Title = {Similarities and differences between electrocardiogram signs of left bundle-branch block and left-ventricular uncoupling},
	Volume = {14},
	Year = {2012}}

@book{rasmussen_gaussian_2006,
	Author = {Rasmussen, C.E. and Williams, C.},
	Publisher = {MIT Press},
	Title = {Gaussian Processes for Machine Learning},
	Year = {2006}}

@article{bilionis_solution_2014,
	Abstract = {Solving inverse problems based on computationally
                   demanding forward models is ubiquitously difficult
                   since one is necessarily limited to just a few
                   observations of the response surface. The usual
                   practice is to replace the response surface with a
                   surrogate. However, this approach induces additional
                   uncertainties on the posterior distributions. The
                   main contribution of this work is the reformulation
                   of the Bayesian solution of the inverse problem when
                   the expensive forward model is replaced by the
                   surrogate. We derive three approximations of the
                   reformulated solution with increasing complexity and
                   fidelity. We demonstrate numerically that the
                   proposed approximations capture the uncertainty of
                   the solution of the inverse problem induced by the
                   fact that the forward model is replaced by a finite
                   number of simulations. We demonstrate our approach in
                   two different problems: locating the contamination
                   source of a diffusive process and inferring the
                   permeability field of an oil reservoir based on
                   measurements of the oil-cut curves.},
	Author = {Bilionis, I. and Zabaras, N.},
	Doi = {10.1088/0266-5611/30/1/015004},
	Issn = {0266-5611},
	Journal = {Inverse Prob.},
	Language = {en},
	Month = jan,
	Number = {1},
	Pages = {015004},
	Title = {Solution of inverse problems with limited forward solver evaluations: a {Bayesian} perspective},
	Url = {http://beta.iopscience.iop.org/0266-5611/30/1/015004},
	Volume = {30},
	Year = {2014},
	Bdsk-Url-1 = {http://beta.iopscience.iop.org/0266-5611/30/1/015004},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/0266-5611/30/1/015004}}

@article{del_moral_sequential_2006,
	Abstract = {We propose a methodology to sample sequentially from
                   a sequence of probability distributions that are
                   defined on a common space, each distribution being
                   known up to a normalizing constant. These probability
                   distributions are approximated by a cloud of weighted
                   random samples which are propagated over time by
                   using sequential {Monte Carlo} methods. This
                   methodology allows us to derive simple algorithms to
                   make parallel Markov chain {Monte Carlo} algorithms
                   interact to perform global optimization and
                   sequential Bayesian estimation and to compute ratios
                   of normalizing constants. We illustrate these
                   algorithms for various integration tasks arising in
                   the context of Bayesian inference.},
	Author = {Del Moral, P. and Doucet, A. and Jasra, A.},
	Doi = {10.1111/j.1467-9868.2006.00553.x},
	Issn = {1369-7412},
	Journal = {Journal of the Royal Statistical Society Series B-Statistical Methodology},
	Language = {English},
	Pages = {411--436},
	Title = {Sequential {Monte} {Carlo} samplers},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1467-9868.2006.00553.x}}

@article{nguyen2015,
	Author = {Nguy{\^e}n, Uy{\^e}n Ch{\^a}u and Potse, Mark and Regoli, Fran{\c{c}}ois and Caputo, Maria Luce and Conte, Giulio and Murzilli, Romina and Muzzarelli, Stefano and Moccetti, Tiziano and Prinzen, Frits W. and Krause, Rolf and Auricchio, Angelo},
	Doi = {10.1016/j.jelectrocard.2015.05.004},
	Journal = {J. Electrocardiol.},
	Month = may,
	Pages = {617-625},
	Title = {An in-silico analysis of the effect of heart position and orientation on the {ECG} morphology and vectorcardiogram parameters in patients with heart failure and intraventricular conduction defects},
	Volume = {48},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.jelectrocard.2015.05.004}}

@article{potse2013,
	Author = {Potse, Mark and Krause, Dorian and Kroon, Wilco and Murzilli, Romina and Muzzarelli, Stefano and Regoli, Fran{\c{c}}ois and Caiani, Enrico and Prinzen, Frits W. and Krause, Rolf and Auricchio, Angelo},
	Doi = {10.1093/europace/euu257},
	Journal = {Europace},
	Pages = {iv56-iv61},
	Title = {Patient-specific modelling of cardiac electrophysiology in heart-failure patients},
	Volume = {16},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/europace/euu257}}

@article{scikit-learn,
	Author = {Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V. and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P. and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
	Journal = {Journal of Machine Learning Research},
	Pages = {2825--2830},
	Title = {Scikit-learn: Machine Learning in {P}ython},
	Volume = {12},
	Year = {2011}}

@book{niederreiter1992random,
	Author = {Niederreiter, Harald},
	Publisher = {SIAM},
	Title = {Random number generation and quasi-{Monte Carlo} methods},
	Year = {1992}}

@book{kalos_monte_2008,
	Abstract = {This introduction to {Monte Carlo} methods seeks to
                   identify and study the unifying elements that
                   underlie their effective application. Initial
                   chapters provide a short treatment of the probability
                   and statistics needed as background, enabling those
                   without experience in {Monte Carlo} techniques to apply
                   these ideas to their research. The book focuses on
                   two basic themes: The first is the importance of
                   random walks as they occur both in natural stochastic
                   systems and in their relationship to integral and
                   differential equations. The second theme is that of
                   variance reduction in general and importance sampling
                   in particular as a technique for efficient use of the
                   methods. Random walks are introduced with an
                   elementary example in which the modeling of radiation
                   transport arises directly from a schematic
                   probabilistic description of the interaction of
                   radiation with matter. Building on this example, the
                   relationship between random walks and integral
                   equations is outlined. The applicability of these
                   ideas to other problems is shown by a clear and
                   elementary introduction to the solution of the
                   Schr{\"\i}¿1⁄2dinger equation by random walks. The
                   text includes sample problems that readers can solve
                   by themselves to illustrate the content of each
                   chapter. This is the second, completely revised and
                   extended edition of the successful monograph, which
                   brings the treatment up to date and incorporates the
                   many advances in {Monte Carlo} techniques and their
                   applications, while retaining the original elementary
                   but general approach.},
	Author = {Kalos, Malvin H. and Whitlock, Paula A.},
	Isbn = {978-3-527-40760-6},
	Language = {en},
	Month = oct,
	Note = {Google-Books-ID: b8Xb4rBkygUC},
	Publisher = {John Wiley \& Sons},
	Title = {Monte {Carlo} {Methods}},
	Year = {2008}}

@incollection{giles_multilevel_2013,
	Author = {Giles, Michael B},
	Booktitle = {Monte {Carlo} and {Quasi}-{Monte} {Carlo} {Methods} 2012},
	Note = {bibtex: giles2013multilevel},
	Pages = {83--103},
	Publisher = {Springer},
	Title = {Multilevel {Monte} {Carlo} methods},
	Year = {2013}}

@book{fishman_monte_2003,
	Address = {New York},
	Author = {Fishman, George},
	Edition = {Corrected edition},
	Isbn = {978-0-387-94527-9},
	Language = {English},
	Month = feb,
	Publisher = {Springer},
	Title = {Monte {Carlo}: Concepts, Algorithms, and Applications},
	Year = {2003}}

@article{diaconis_bayesian_1988,
	Author = {Diaconis, Persi},
	Journal = {Statistical decision theory and related topics IV},
	Pages = {163--175},
	Title = {Bayesian numerical analysis},
	Volume = {1},
	Year = {1988}}

@article{ohagan_monte_1987,
	Abstract = {We present some fundamental objections to the Monte
                   Carlo method of numerical integration.},
	Author = {O'Hagan, A.},
	Doi = {10.2307/2348519},
	Issn = {0039-0526},
	Journal = {Journal of the Royal Statistical Society. Series D (The Statistician)},
	Number = {2/3},
	Pages = {247--249},
	Title = {Monte {Carlo} is Fundamentally Unsound},
	Url = {http://www.jstor.org/stable/2348519},
	Volume = {36},
	Year = {1987},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2348519},
	Bdsk-Url-2 = {http://dx.doi.org/10.2307/2348519}}

@article{ohagan_bayes-hermite_1991,
	Author = {O'Hagan, A},
	Journal = {Journal of statistical planning and inference},
	Number = {3},
	Optnote = {bibtex: o1991bayes},
	Pages = {245--260},
	Title = {Bayes-{Hermite} quadrature},
	Volume = {29},
	Year = {1991}}

@inproceedings{rasmussen_bayesian_2003,
	Author = {Rasmussen, C. E. and Ghahramani, Z.},
	Booktitle = {Advances in {Neural} {Information} {Processing} {Systems} 15},
	Publisher = {MIT Press},
	Title = {Bayesian {Monte} {Carlo}},
	Year = {2003}}

@article{conti_bayesian_2010,
	Abstract = {Computer models are widely used in scientific
                   research to study and predict the behaviour of
                   complex systems. The run times of computer-intensive
                   simulators are often such that it is impractical to
                   make the thousands of model runs that are
                   conventionally required for sensitivity analysis.
                   uncertainty analysis or calibration. In response to
                   this problem, highly efficient techniques have
                   recently been developed based on a statistical
                   meta-model (the emulator) that is built to
                   approximate the computer model. The approach,
                   however, is less straightforward for dynamic
                   simulators. designed to represent time-evolving
                   systems. Generalisations of the established
                   methodology to allow for dynamic emulation are here
                   proposed and contrasted. Advantages and difficulties
                   are discussed and illustrated with an application to
                   the Sheffield Dynamic Global Vegetation Model,
                   developed within the UK Centre for Terrestrial Carbon
                   Dynamics. (C) 2009 Elsevier B.V. All rights
                   reserved.},
	Annote = {WOS:000272635800005},
	Author = {Conti, Stefano and O'Hagan, Anthony},
	Doi = {10.1016/j.jspi.2009.08.006},
	Journal = {Journal of Statistical Planning and Inference},
	Month = mar,
	Number = {3},
	Pages = {640--651},
	Title = {Bayesian emulation of complex multi-output and dynamic computer models},
	Volume = {140},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.jspi.2009.08.006}}

@book{papoulis_probability_2002,
	Abstract = {The fourth edition of Probability, Random Variables
                   and Stochastic Processes has been updated
                   significantly from the previous edition, and it now
                   includes co-author S. Unnikrishna Pillai of
                   Polytechnic University. The book is intended for a
                   senior/graduate level course in probability and is
                   aimed at students in electrical engineering, math,
                   and physics departments. The authors' approach is to
                   develop the subject of probability theory and
                   stochastic processes as a deductive discipline and to
                   illustrate the theory with basic applications of
                   engineering interest. Approximately 1/3 of the text
                   is new material--this material maintains the style
                   and spirit of previous editions. In order to bridge
                   the gap between concepts and applications, a number
                   of additional examples have been added for further
                   clarity, as well as several new topics.},
	Address = {Boston, Mass.},
	Author = {Papoulis, Athanasios and Pillai, S. Unnikrishna},
	Edition = {4th edition},
	Isbn = {978-0-07-122661-5},
	Language = {English},
	Month = jan,
	Publisher = {McGraw-Hill Europe},
	Title = {Probability, Random Variables and Stochastic Processes},
	Year = {2002}}

@book{gian,
	Author = {Hesthaven, Jan S. and Rozza, Gianluigi and Stamm, Benjamin and others},
	Doi = {10.1007/978-3-319-22470-1},
	Publisher = {Springer},
	Title = {Certified reduced basis methods for parametrized partial differential equations},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/978-3-319-22470-1}}

@article{henriquez14,
	Author = {Henriquez, Craig S.},
	Journal = {IEEE Trans. Biomed. Eng.},
	Pages = {1457-1465},
	Title = {A Brief History of Tissue Models For Cardiac Electrophysiology},
	Volume = {61},
	Year = {2014}}

@article{Chabiniok2016,
	Abstract = {With heart and cardiovascular diseases continually challenging healthcare systems worldwide, translating basic research on cardiac (patho)physiology into clinical care is essential. Exacerbating this already extensive challenge is the complexity of the heart, relying on its hierarchical structure and function to maintain cardiovascular flow. Computational modelling has been proposed and actively pursued as a tool for accelerating research and translation. Allowing exploration of the relationships between physics, multiscale mechanisms and function, computational modelling provides a platform for improving our understanding of the heart. Further integration of experimental and clinical data through data assimilation and parameter estimation techniques is bringing computational models closer to use in routine clinical practice. This article reviews developments in computational cardiac modelling and how their integration with medical imaging data is providing new pathways for translational cardiac modelling.},
	Author = {Chabiniok, Radomir and Wang, Vicky Y. and Hadjicharalambous, Myrianthi and Asner, Liya and Lee, Jack and Sermesant, Maxime and Kuhl, Ellen and Young, Alistair A. and Moireau, Philippe and Nash, Martyn P. and Chapelle, Dominique and Nordsletten, David A.},
	Doi = {10.1098/rsfs.2015.0083},
	File = {:Users/peppu/work/articoli/altri/chabiniok2016.pdf:pdf},
	Issn = {2042-8898},
	Journal = {Interface Focus},
	Keywords = {biomechanics,biomedical engineering,mathematical physics heart},
	Number = {2},
	Pages = {20150083},
	Pmid = {27051509},
	Title = {{Multiphysics and multiscale modelling, data--model fusion and integration of organ physiology in the clinic: ventricular cardiac mechanics}},
	Url = {http://rsfs.royalsocietypublishing.org/lookup/doi/10.1098/rsfs.2015.0083},
	Volume = {6},
	Year = {2016},
	Bdsk-Url-1 = {http://rsfs.royalsocietypublishing.org/lookup/doi/10.1098/rsfs.2015.0083},
	Bdsk-Url-2 = {http://dx.doi.org/10.1098/rsfs.2015.0083}}

@article{Lamata2013,
	Author = {Lamata, Pablo and Sinclair, Matthew and Kerfoot, Eric and Lee, Angela and Crozier, Andrew and Blazevic, Bojan and Land, Sander and Lewandowski, Adam J and Barber, David and Niederer, Steve and Smith, Nic},
	Doi = {10.1098/rsif.2013.1023},
	File = {:Users/peppu/work/articoli/altri/lamata2016.pdf:pdf},
	Issn = {1742-5689},
	Journal = {Journal of The Royal Society Interface},
	Keywords = {biomechanics,biomedical engineering},
	Month = {dec},
	Number = {91},
	Pages = {20131023},
	Title = {{An automatic service for the personalization of ventricular cardiac meshes}},
	Url = {http://rsif.royalsocietypublishing.org/cgi/doi/10.1098/rsif.2013.1023},
	Volume = {11},
	Year = {2013},
	Bdsk-Url-1 = {http://rsif.royalsocietypublishing.org/cgi/doi/10.1098/rsif.2013.1023},
	Bdsk-Url-2 = {http://dx.doi.org/10.1098/rsif.2013.1023}}

@article{Xia2015,
	Abstract = {Large-scale 3D virtual heart model simulations are highly demanding in computational resources. This imposes a big challenge to the traditional computation resources based on CPU environment, which already cannot meet the requirement of the whole computation demands or are not easily available due to expensive costs. GPU as a parallel computing environment therefore provides an alternative to solve the large-scale computational problems of whole heart modeling. In this study, using a 3D sheep atrial model as a test bed, we developed a GPU-based simulation algorithm to simulate the conduction of electrical excitation waves in the 3D atria. In the GPU algorithm, a multicellular tissue model was split into two components: one is the single cell model (ordinary differential equation) and the other is the diffusion term of the monodomain model (partial differential equation). Such a decoupling enabled realization of the GPU parallel algorithm. Furthermore, several optimization strategies were proposed based on the features of the virtual heart model, which enabled a 200-fold speedup as compared to a CPU implementation. In conclusion, an optimized GPU algorithm has been developed that provides an economic and powerful platform for 3D whole heart simulations.},
	Author = {Xia, Yong and Wang, Kuanquan and Zhang, Henggui},
	Doi = {10.1155/2015/862735},
	File = {:Users/peppu/work/articoli/altri/xia2015.pdf:pdf},
	Issn = {17486718},
	Journal = {Comput. Math. Methods Med.},
	Title = {Parallel Optimization of {3D} Cardiac Electrophysiological Model Using {GPU}},
	Volume = {2015},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1155/2015/862735}}

@article{avo11,
	Author = {van Oosterom, Adriaan and Oostendorp, Thom F. and van Dam, Peter M.},
	Journal = {J. Electrocardiol.},
	Pages = {577-583},
	Title = {Potential applications of the new {ECGSIM}},
	Volume = {44},
	Year = {2011}}

@article{Clayton2011,
	Author = {R.H. Clayton and O. Bernus and E.M. Cherry and H. Dierckx and F.H. Fenton and L. Mirabella and A.V. Panfilov and F.B. Sachse and G. Seemann and H. Zhang},
	Issn = {0079-6107},
	Journal = {Prog. Biophys. Mol. Biol.},
	Number = {1-3},
	Pages = {22-48},
	Title = {Models of cardiac tissue electrophysiology: Progress, challenges and open questions},
	Volume = {104},
	Year = {2011}}

@inproceedings{dkrause11a,
	Address = {Berlin},
	Author = {Krause, Dorian and Potse, Mark and Dickopf, Thomas and Krause, Rolf and Auricchio, Angelo and Prinzen, Frits W.},
	Booktitle = {Facing the Multicore-Challenge II},
	Editor = {Keller, Rainer and Kramer, David and Weiss, Jan-Philipp},
	Pages = {120-132},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Tags = {mpcvproceedings},
	Title = {Hybrid Parallelization of a Large-Scale Heart Model},
	Volume = {7174},
	Year = {2012}}

@article{Erem2014,
	Author = {Erem, Burak and van Dam, Peter and Brooks, Dana H.},
	Doi = {10.1109/tmi.2014.2297952},
	Journal = {{IEEE} Transactions on Medical Imaging},
	Month = {apr},
	Number = {4},
	Pages = {902-912},
	Publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
	Title = {Identifying Model Inaccuracies and Solution Uncertainties in Noninvasive Activation-Based Imaging of Cardiac Excitation Using Convex Relaxation},
	Volume = {33},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1109/tmi.2014.2297952}}

@article{Trayanova2011,
	Author = {Trayanova, Natalia A},
	Doi = {10.1161/CIRCRESAHA.110.223610},
	Issn = {0009-7330},
	Journal = {Circ. Res.},
	Month = {jan},
	Number = {1},
	Pages = {113--128},
	Publisher = {Am Heart Assoc},
	Title = {Whole-Heart Modeling: Applications to Cardiac Electrophysiology and Electromechanics},
	Url = {http://circres.ahajournals.org/cgi/doi/10.1161/CIRCRESAHA.110.223610},
	Volume = {108},
	Year = {2011},
	Bdsk-Url-1 = {http://circres.ahajournals.org/cgi/doi/10.1161/CIRCRESAHA.110.223610},
	Bdsk-Url-2 = {http://dx.doi.org/10.1161/CIRCRESAHA.110.223610}}

@article{pezzuto2016,
	Author = {Pezzuto, Simone and Hake, Johan and Sundnes, Joakim},
	Doi = {10.1002/cnm.2762},
	Journal = {Int. J. Numer. Meth. Biomed. Engng.},
	Title = {Space-discretization error analysis and stabilization schemes for conduction velocity in cardiac electrophysiology},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/cnm.2762}}

@book{Katz2010,
	Author = {Katz, Arnold M},
	Publisher = {Lippincott Williams \& Wilkins},
	Title = {Physiology of the Heart},
	Year = {2010}}

@article{Villongco2014,
	Abstract = {Patient-specific computational models have promise to improve cardiac disease diagnosis and therapy planning. Here a new method is described to simulate left-bundle branch block (LBBB) and RV-paced ventricular activation patterns in three dimensions from non-invasive, routine clinical measurements. Activation patterns were estimated in three patients using vectorcardiograms (VCG) derived from standard 12-lead electrocardiograms (ECG). Parameters of a monodomain model of biventricular electrophysiology were optimized to minimize differences between the measured and computed VCG. Electroanatomic maps of local activation times measured on the LV and RV endocardial surfaces of the same patients were used to validate the simulated activation patterns. For all patients, the optimal estimated model parameters predicted a time-averaged mean activation dipole orientation within 6.7$\pm$0.6$\,^{\circ}$ of the derived VCG. The predicted local activation times agreed within 11.5$\pm$0.8ms of the measured electroanatomic maps, on the order of the measurement accuracy.},
	Author = {Villongco, Christopher T. and Krummen, David E. and Stark, Paul and Omens, Jeffrey H. and McCulloch, Andrew D.},
	Doi = {10.1016/j.pbiomolbio.2014.06.011},
	File = {:Users/peppu/work/articoli/altri/villongco2014.pdf:pdf},
	Issn = {00796107},
	Journal = {Progress in Biophysics and Molecular Biology},
	Keywords = {Monodomain model,Patient-specific model,Vectorcardiogram},
	Number = {2-3},
	Pages = {305--313},
	Pmid = {25110279},
	Publisher = {Elsevier Ltd},
	Title = {{Patient-specific modeling of ventricular activation pattern using surface ECG-derived vectorcardiogram in bundle branch block}},
	Url = {http://dx.doi.org/10.1016/j.pbiomolbio.2014.06.011},
	Volume = {115},
	Year = {2014},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.pbiomolbio.2014.06.011}}

@article{tusscher04,
	Author = {ten Tusscher, K. H. W. J. and Noble, D. and Noble, P. J. and Panfilov, A. V.},
	Journal = {Am. J. Physiol. Heart Circ. Physiol.},
	Mp_Idx = {656},
	Mp_Topics = {models membrane},
	Pages = {H1573--H1589},
	Title = {A model for human ventricular tissue},
	Volume = {286},
	Year = {2004}}

@article{Tusscher2006,
	Author = {K. H. W. J. ten Tusscher and A. V. Panfilov},
	Doi = {10.1152/ajpheart.00109.2006},
	Journal = {American Journal of Physiology-Heart and Circulatory Physiology},
	Month = {sep},
	Number = {3},
	Pages = {H1088--H1100},
	Publisher = {Am Physiological Soc},
	Title = {Alternans and spiral breakup in a human ventricular tissue model},
	Volume = {291},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1152/ajpheart.00109.2006}}

@book{Stru1899a,
		Author = {William Strunk and E. B. White},
		Title = {The Elements of Style},
		Edition = {4th},
		ISBN = {0-205-30902-X},
		Keywords = {},
		Publisher = {Longman Publishers},
		Year = {1899}}
		
		
		
@article{harbrecht2015efficient,
  title={Efficient approximation of random fields for numerical applications},
  author={Harbrecht, Helmut and Peters, Michael and Siebenmorgen, Markus},
  journal={Numerical Linear Algebra with Applications},
  volume={22},
  number={4},
  pages={596--617},
  year={2015},
  publisher={Wiley Online Library}
}

@article{gander2016analysis,
  title={Analysis of a new space-time parallel multigrid algorithm for parabolic problems},
  author={Gander, Martin J. and Neum\"uller, Martin},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  number={4},
  pages={A2173--A2208},
  year={2016},
  publisher={SIAM}
}

@incollection{giles2013multilevel,
  title={Multilevel {Monte Carlo} methods},
  author={Giles, Michael B},
  booktitle={{Monte Carlo} and Quasi-{Monte Carlo} Methods 2012},
  pages={83--103},
  year={2013},
  publisher={Springer}
}

@article{hodgkin1952quantitative,
  title={A quantitative description of membrane current and its application to conduction and excitation in nerve},
  author={Hodgkin, Alan L. and Huxley, Andrew F.},
  journal={The Journal of physiology},
  volume={117},
  number={4},
  pages={500--544},
  year={1952},
  publisher={Wiley Online Library}
}

@article{hurtado2014gradient,
  title={Gradient flows and variational principles for cardiac electrophysiology: toward efficient and robust numerical simulations of the electrical activity of the heart},
  author={Hurtado, Daniel E. and Henao, Duvan},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={273},
  pages={238--254},
  year={2014},
  publisher={Elsevier}
}

@article{miller1978simulation,
  title={Simulation studies of the electrocardiogram. I. The normal heart.},
  author={Miller, Walter T. and Geselowitz, David B.},
  journal={Circulation Research},
  volume={43},
  number={2},
  pages={301--315},
  year={1978},
  publisher={Am Heart Assoc}
}

@misc{Zulian2017d,
    author = {Patrick Zulian and Alena Kopani{\v c}{\'a}kov{\'a} and Maria Chiara Giuseppina Nestola and Andreas Fink and Nur Fadel and Victor Magri and Teseo Schneider and Eric Botter and Jan Mankau and Rolf Krause},
    title = {{U}topia: {A} {C}++ embedded domain specific language for scientific computing},
    url = {https://bitbucket.org/zulianp/utopia},
    howpublished = {software},
    year = {2016}
}

@misc{quaglino2017h,
Author = {Quaglino, Alessio and Ben Bader, Seif and Krause, Rolf},
Date-Added = {2018-04-19 08:00:15 +0000},
Date-Modified = {2018-04-19 08:01:15 +0000},
Howpublished = {software},
Title = {{SLOTH: An opensource Python library for UQ, available at https://bitbucket.org/quagla/sloth/src/master/}},
Year = {2017}
}

@misc{osti_1231725,
title = {Multiphysics Object Oriented Simulation Environment ({MOOSE}) },
author = {},
abstractNote = {The Multiphysics Object Oriented Simulation Environment (MOOSE) software library developed at Idaho National Laboratory is a tool. MOOSE, like other tools, doesn't actually complete a task. Instead, MOOSE seeks to reduce the effort required to create engineering simulation applications. MOOSE itself is a software library: a blank canvas upon which you write equations and then MOOSE can help you solve them. MOOSE is comparable to a spreadsheet application. A spreadsheet, by itself, doesn't do anything. Only once equations are entered into it will a spreadsheet application compute anything. Such is the same for MOOSE. An engineer or scientist can utilize the equation solvers within MOOSE to solve equations related to their area of study. For instance, a geomechanical scientist can input equations related to water flow in underground reservoirs and MOOSE can solve those equations to give the scientist an idea of how water could move over time. An engineer might input equations related to the forces in steel beams in order to understand the load bearing capacity of a bridge. Because MOOSE is a blank canvas it can be useful in many scientific and engineering pursuits.},
url = {https://www.osti.gov//servlets/purl/1231725},
doi = {},
year = {2014},
month = {2},
 
}

@article{drzisga2017scheduling,
  title={Scheduling massively parallel multigrid for multilevel {Monte Carlo} methods},
  author={Drzisga, Daniel and Gmeiner, Bj{\"o}rn and Rüde, U. and Scheichl, Robert and Wohlmuth, Barbara I.},
  journal={SIAM Journal on Scientific Computing},
  volume={39},
  number={5},
  pages={S873--S897},
  year={2017},
  publisher={SIAM}
}


@article{krause2016enabling,
  title={Enabling local time stepping in the parallel implicit solution of reaction--diffusion equations via space-time finite elements on shallow tree meshes},
  author={Krause, Dorian and Krause, Rolf},
  journal={Applied Mathematics and Computation},
  volume={277},
  pages={164--179},
  year={2016},
  publisher={Elsevier}
}

@article{horton1995space,
  title={A space-time multigrid method for parabolic partial differential equations},
  author={Horton, Graham and Vandewalle, Stefan},
  journal={SIAM Journal on Scientific Computing},
  volume={16},
  number={4},
  pages={848--864},
  year={1995},
  publisher={SIAM}
}

@book{dennis1996numerical,
  title={Numerical methods for unconstrained optimization and nonlinear equations},
  author={Dennis Jr, John E and Schnabel, Robert B},
  volume={16},
  year={1996},
  publisher={Siam}
}

@article{pullan2002finite,
  title={A finite element method for an eikonal equation model of myocardial excitation wavefront propagation},
  author={Pullan, Andrew J and Tomlinson, Karl A and Hunter, Peter J},
  journal={SIAM Journal on Applied Mathematics},
  volume={63},
  number={1},
  pages={324--350},
  year={2002},
  publisher={SIAM}
}

@article{franzone1993spreading,
  title={Spreading of excitation in 3-d models of the anisotropic cardiac tissue. I. Validation of the eikonal model},
  author={Franzone, Piero Colli and Guerri, Luciano},
  journal={Mathematical biosciences},
  volume={113},
  number={2},
  pages={145--209},
  year={1993},
  publisher={Elsevier}
}

@article{fitzhugh1961impulses,
  title={Impulses and physiological states in theoretical models of nerve membrane},
  author={FitzHugh, Richard},
  journal={Biophysical journal},
  volume={1},
  number={6},
  pages={445--466},
  year={1961},
  publisher={Elsevier}
}

@article{speck2014space,
  title={A space-time parallel solver for the three-dimensional heat equation},
  author={Speck, Robert and Ruprecht, Daniel and Emmett, Matthew and Bolten, Matthias and Krause, Rolf},
  journal={Parallel Computing: Accelerating Computational Science and Engineering (CSE)},
  volume={25},
  pages={263--272},
  year={2014},
  publisher={IOS Press}
}

@article{franco2018multigrid,
  title={Multigrid method based on a space-time approach with standard coarsening for parabolic problems},
  author={Franco, Sebasti{\~a}o Romero and Gaspar, Francisco Jos{\'e} and Pinto, Marcio Augusto Villela and Rodrigo, Carmen},
  journal={Applied Mathematics and Computation},
  volume={317},
  pages={25--34},
  year={2018},
  publisher={Elsevier}
}

@Article{Falgout2017,
author="Falgout, R. D.
and Friedhoff, S.
and Kolev, Tz. V.
and MacLachlan, S. P.
and Schroder, J. B.
and Vandewalle, S.",
title="Multigrid methods with space--time concurrency",
journal="Computing and Visualization in Science",
year="2017",
month="Aug",
day="01",
volume="18",
number="4",
pages="123--143",
doi="10.1007/s00791-017-0283-9",
url="https://doi.org/10.1007/s00791-017-0283-9"
}
 

@inproceedings{Hackbusch:1985,
 author = {Hackbusch, Wolfgang},
 title = {Parabolic Multi-grid Methods},
 booktitle = {Proc. Of the Sixth Int'L. Symposium on Computing Methods in Applied Sciences and Engineering, VI},
 year = {1985},
 isbn = {0-444-87597-2},
 location = {Versailles, France},
 pages = {189--197},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=4673.4714},
 acmid = {4714},
 publisher = {North-Holland Publishing Co.},
 address = {Amsterdam, The Netherlands, The Netherlands},
} 

@article{quaglino2019high,
  title={High-dimensional and higher-order multifidelity {Monte Carlo} estimators},
  author={Quaglino, Alessio and Pezzuto, Simone and Krause, Rolf},
  journal={Journal of Computational Physics},
  volume={388},
  pages={300--315},
  year={2019},
  publisher={Elsevier}
}


@article{charrier2013finite,
  title={Finite element error analysis of elliptic {PDE}s with random coefficients and its application to multilevel {Monte Carlo} methods},
  author={Charrier, Julia and Scheichl, Robert and Teckentrup, Aretha L.},
  journal={SIAM Journal on Numerical Analysis},
  volume={51},
  number={1},
  pages={322--352},
  year={2013},
  publisher={SIAM}
}

@article{teckentrup2013further,
  title={Further analysis of multilevel {Monte Carlo} methods for elliptic {PDE}s with random coefficients},
  author={Teckentrup, Aretha L. and Scheichl, Robert and Giles, Michael B. and Ullmann, Elisabeth},
  journal={Numerische Mathematik},
  volume={125},
  number={3},
  pages={569--600},
  year={2013},
  publisher={Springer}
}

@incollection{harbrecht2012multilevel,
  title={On multilevel quadrature for elliptic stochastic partial differential equations},
  author={Harbrecht, Helmut and Peters, Michael and Siebenmorgen, Markus},
  booktitle={Sparse grids and applications},
  pages={161--179},
  year={2012},
  publisher={Springer}
}

@article{barth2011multi,
  title={Multi-level {Monte Carlo} finite element method for elliptic {PDE}s with stochastic coefficients},
  author={Barth, Andrea and Schwab, Christoph and Zollinger, Nathaniel},
  journal={Numerische Mathematik},
  volume={119},
  number={1},
  pages={123--161},
  year={2011},
  publisher={Springer}
}

@book{quarteroni2010numerical,
  title={Numerical mathematics},
  author={Quarteroni, Alfio and Sacco, Riccardo and Saleri, Fausto},
  volume={37},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@article{french1993analysis,
  title={Analysis of a robust finite element approximation for a parabolic equation with rough boundary data},
  author={French, Donald A. and King, J. Thomas},
  journal={Mathematics of computation},
  volume={60},
  number={201},
  pages={79--104},
  year={1993}
}

@article{gong2013error,
  title={Error estimates for parabolic optimal control problems with control and state constraints},
  author={Gong, Wei and Hinze, Michael},
  journal={Computational Optimization and Applications},
  volume={56},
  number={1},
  pages={131--151},
  year={2013},
  publisher={Springer}
}

@article{aziz1989continuous,
  title={Continuous finite elements in space and time for the heat equation},
  author={Aziz, Kadir A. and Monk, Peter},
  journal={Mathematics of Computation},
  volume={52},
  number={186},
  pages={255--274},
  year={1989}
}

@article{bonizzoni2014moment,
  title={Moment equations for the mixed formulation of the {Hodge Laplacian} with stochastic loading term},
  author={Bonizzoni, Francesca and Buffa, Annalisa and Nobile, Fabio},
  journal={IMA Journal of Numerical Analysis},
  volume={34},
  number={4},
  pages={1328--1360},
  year={2014},
  publisher={OUP}
}

@article{kreuter2015sobolev,
  title={Sobolev spaces of vector-valued functions},
  author={Kreuter, Marcel},
  journal={Ulm University Faculty of Mathematics and Economies},
  year={2015}
}

@TechReport{petsc-user-ref,
  Author = {Satish Balay and Shrirang Abhyankar and Mark F. Adams and Jed Brown and Peter Brune
            and Kris Buschelman and Lisandro Dalcin and Victor Eijkhout and William D. Gropp
            and Dinesh Kaushik and Matthew G. Knepley
            and Lois Curfman McInnes and Karl Rupp and Barry F. Smith
            and Stefano Zampini and Hong Zhang and Hong Zhang},
  Title = {{PETS}c Users Manual},
  Number = {ANL-95/11 - Revision 3.7},
  Institution = {Argonne National Laboratory},
  Year = {2016}
}

@article{Benedusi2018,
  title={Space-Time {FE-DG} Discretization of the Anisotropic Diffusion Equation in Any Dimension: the Spectral Symbol},
  author={Benedusi, Pietro and Garoni, Carlo and Krause, Rolf and Li, Xiaozhou and Serra-Capizzano, Stefano},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={39},
  number={3},
  pages={1383--1420},
  year={2018},
  publisher={SIAM}
}

@incollection{gander201550,
  title={50 years of time parallel time integration},
  author={Gander, Martin J.},
  booktitle={Multiple Shooting and Time Domain Decomposition Methods},
  pages={69--113},
  year={2015},
  publisher={Springer}
}


@article{gander2016analysis,
  title={Analysis of a new space-time parallel multigrid algorithm for parabolic problems},
  author={Gander, Martin J and Neumuller, Martin},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  number={4},
  pages={A2173--A2208},
  year={2016},
  publisher={SIAM}
}

@incollection{mcdonald2016simple,
  title={A simple proposal for parallel computation over time of an evolutionary process with implicit time stepping},
  author={McDonald, Eleanor and Wathen, Andy},
  booktitle={Numerical Mathematics and Advanced Applications ENUMATH 2015},
  pages={285--293},
  year={2016},
  publisher={Springer}
}

@article{krause2016parallel,
  title={A parallel approach to the variational transfer of discrete fields between arbitrarily distributed unstructured finite element meshes},
  author={Krause, Rolf and Zulian, Patrick},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  number={3},
  pages={C307--C333},
  year={2016},
  publisher={SIAM}
}

@article{quaglino2018fast,
  title={Fast uncertainty quantification of activation sequences in patient-specific cardiac electrophysiology meeting clinical time constraints},
  author={Quaglino, Alessio and Pezzuto, Simone and Koutsourelakis, Phaedon-Stelios  and Auricchio, Angelo and Krause, Rolf},
  journal={International journal for numerical methods in biomedical engineering},
  volume={34},
  number={7},
  pages={e2985},
  year={2018},
  publisher={Wiley Online Library}
}

@article{wohlmuth_2000,
  title={A mortar finite element method using dual spaces for the Lagrange multiplier},
  author={Wohlmuth, Barbara I.},
  journal={SIAM journal on numerical analysis},
  volume={38},
  number={3},
  pages={989--1012},
  year={2000},
  publisher={SIAM}
}

@article{popp_2012,
  title={Dual quadratic mortar finite element methods for {3D} finite deformation contact},
  author={Popp, Alexander and Wohlmuth, Barbara I. and Gee, Michael W. and Wall, Wolfgang A.},
  journal={SIAM Journal on Scientific Computing},
  volume={34},
  number={4},
  pages={B421--B446},
  year={2012},
  publisher={SIAM}
}

@article{hesch,
author = {Hesch, Christian and Betsch, Peter},
title = {A comparison of computational methods for large deformation contact problems of flexible bodies},
journal = {ZAMM - Journal of Applied Mathematics and Mechanics / Zeitschrift f{\"u}r Angewandte Mathematik und Mechanik},
volume = {86},
number = {10},
year = {2006},
pages = {818--827},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/zamm.200610289}
}

@article{nievergelt1964parallel,
  title={Parallel methods for integrating ordinary differential equations},
  author={Nievergelt, J{\"u}rg},
  journal={Communications of the ACM},
  volume={7},
  number={12},
  pages={731--733},
  year={1964},
  publisher={ACM}
}


